Grow and Merge: A Unified Framework for Continuous Categories Discovery

Although a number of studies are devoted to novel category discovery, most of them assume a static setting where both labeled and unlabeled data are given at once for finding new categories. In this work, we focus on the application scenarios where unlabeled data are continuously fed into the category discovery system. We refer to it as the {\bf Continuous Category Discovery} ({\bf CCD}) problem, which is significantly more challenging than the static setting. A common challenge faced by novel category discovery is that different sets of features are needed for classification and category discovery: class discriminative features are preferred for classification, while rich and diverse features are more suitable for new category mining. This challenge becomes more severe for dynamic setting as the system is asked to deliver good performance for known classes over time, and at the same time continuously discover new classes from unlabeled data. To address this challenge, we develop a framework of {\bf Grow and Merge} ({\bf GM}) that works by alternating between a growing phase and a merging phase: in the growing phase, it increases the diversity of features through a continuous self-supervised learning for effective category mining, and in the merging phase, it merges the grown model with a static one to ensure satisfying performance for known classes. Our extensive studies verify that the proposed GM framework is significantly more effective than the state-of-the-art approaches for continuous category discovery.

==> NeurIPS 2022 SMNet_0517_arxiv/checklist.tex <==
\section*{Checklist}



\begin{enumerate}


\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{} See supplementary materials.
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{} See supplementary materials.
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}


\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{} Theoretical results are not included.
        \item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}


\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{} See the supplementary materials.
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{} See section~\ref{sec:exp} and supplementary materials.
        \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerNo{}
        \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{} See supplementary materials.
\end{enumerate}


\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{} See Section~\ref{sec:exp}.
  \item Did you mention the license of the assets?
    \answerNA{} The license of the assets are not provided on their official website.
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNo{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNo{}
\end{enumerate}


\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{} Crowdsourcing and human subjects are not used in this research.
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}


\end{enumerate}

==> NeurIPS 2022 SMNet_0517_arxiv/sections/chap01_introduction.tex <==
\section{Introduction}

% 1.	研究背景、意义，介绍无监督增量应用场景
% 2.	其他方法的不足
% 3.	挑战：遗忘、挖掘
% 4.    贡献

% 【新类挖掘任务】
% 人类的视觉认知是以对物体的语义分类为基础的，而类别的定义则是随着历史的发展和知识的积累逐渐完善和更新的。在当今的视觉智能体研究中，我们不仅训练机器学会人类的分类行为（引用），更希望其掌握人类通过现有知识定义新类别的能力，使其能够自主进化和学习（引用）。这一行为在近期工作中被定义为“新类挖掘”，且取得了不错的从无标签数据中聚类和定义新类别的效果。
Human beings are good at grouping objects into category through clustering, and the definition of categories are continuously expanding and updated over time. 
Recent developments of intelligent visual systems can not only distinguish pre-defined categories~\cite{DBLP:conf/eccv/GansbekeVGPG20, DBLP:conf/nips/BerthelotCGPOR19, simclr, moco,feng2022rethinking}, but also discover new categories from unlabeled data, a task that is known as \textit{novel category discovery}~\cite{han2021autonovel, UNO, DBLP:journals/corr/abs-2201-02609}.  

% 【现有设置问题（真实场景）】
% 现有的新类挖掘工作是通常建立在单阶段场景下的，即所有的有标签和无标签数据同时给出。在此场景下，已有方法先进行有监督或半监督表征学习，再在无标签数据上进行聚类挖掘，取得了不错的效果。然而，这种单阶段设置与实际的应用场景有着很大的区别：1.真实场景下无标签数据往往是增量出现的，特别是在模型已经在有标签数据上完成训练并上线使用后；2.真实应用中是无法获取纯未知类别的数据的，通常输入的是无标签的已知和未知类别数据的混合；3.当前设置仅关注新类挖掘的效果，但忽视了新类挖掘和记忆过程对于旧类分类性能的损坏，这对于实际使用场景是不可接受的。
Existing works on novel category discovery are limited to the \textit{static} setting, where both labeled data (by known classes) and unlabeled data (with potential unknown categories) are given at once. In contrast, for real-world applications, unlabeled data are continuously fed into the system for discovering new categories, making it a significantly more challenging problem. Besides, current studies for novel category discovery often assume that all the unlabeled data belong to the unknown new categories, which is generally not true in real applications. In this work, we examine the dynamic setup of novel category discovery where the system was initially given a set of data labeled by known classes, and unlabeled data are continuously streamed into the system for discovering new classes. The system is requested to consistently yield satisfying performance for known classes, and at the same time, dynamically discover new categories from the streaming unlabeled data. We refer to it as {\bf Continuous Category Discovery}, or {\bf CCD} for short.    




% (iii) The single-stage scenario mainly concentrates on the performance of category discovery, while neglects its damage on the performance of classifying previously known categories.

% 【框架定义】
%To address the above problems, in this paper, we study the \textbf{Incremental Novel Category Discovery (CCD)}.
%The input of CCD is a continuous data stream containing both labeled and unlabeled data from known and unknown categories. 
%At each time-step, there are two main tasks: (i) discovering newly-appeared novel categories and merging them into the known category set of current model, (ii) alleviating the forgetting of classification on previously known categories.

% A qualified method under such a scenario should own the following abilities: (i) maintaining classification performance on currently known categories or with acceptable forgetting, (ii) distinguishing known and unknown categories from the unlabeled incremental data, (iii) discovering novel categories and merging them into the known categories of current model. 
% 这个图应该用示意的形式，把当前已知类别、输入数据的有无标签和是否新类等表示出来，展示连续挖掘过程。
We illustrate the process of CCD in Figure~\ref{fig:setting}. It is comprised of two main stages: the \textit{initial stage} where a classification model is trained by a set of labeled examples, and the \textit{continuous category discovery stage} where new categories are continuously discovered from a stream of unlabeled data belonging to both known and unknown classes. A intuitive approach to address the dynamic nature of CCD is to combine the existing methods for open-set recognition~\cite{osr,osrsurvey, DBLP:conf/iccv/Wu0JMTL21}, novel category discovery~\cite{han2020automatically, han2021autonovel, dtc}, and incremental learning~\cite{lwf, icarl}. %(see section~\ref{sec_rel} for details). 
This is however insufficient because our learning system has to accomplish two tasks at the same time, \ie, accurately classify instances into the known classes, and discover new categories from an unlabeled data stream. It turns out that these two task models usually produce different types of features: discriminative features on known classes are preferred by classification model, while rich and diverse features are critical for identifying new classes, as illustrated in Figure~\ref{fig:features}. A simple combination of novel category discovery and incremental learning will fail to address the trade-off consistently over time, which is further verified by our empirical studies.   

\begin{figure}[htbp]
  \centering
  \includegraphics[width=0.9\linewidth]{imgs/setting.pdf}
  \caption{\textbf{Overview of the Continuous Category Discovery (CCD).} The continuous data stream is mixed with unlabeled samples from both known and novel categories. CCD requires to distinguish known categories, discover novel categories and merge the discovered categories into known set.}
  \label{fig:setting}
\end{figure}



To address the challenge of continuous category discovery, we propose a framework of {\bf Grow} and {\bf Merge}, or {\bf GM} for short. After pre-training a static model $\mathcal{A}$ over the labeled data, we will update model $\mathcal{A}$ with respect to unlabeled data stream by alternating between the growing phase and the merging phase: in the growing phase, we will increase the diversity of features by continuously training our model over received unlabeled data through a combination of supervised and self-supervised learning; in the merging phase, we will merge the grown model with the static one by taking a weighted combination of both models. By alternating between the growing and merging phases, we are able to maintain a good performance for known classes, and at same time, the power of discovering new categories. This is clearly visualized in Figure~\ref{fig:features}, where the first two panels show that existing approaches can do well on one of the two tasks but not both, and last panel shows that features learned by the proposed GM framework works well for both tasks. 

Finally, one of the common issues with continuous training is catastrophic forgetting. To alleviating the forgetting effect as we are growing the number of categories over time, 
we maintain a small set of labeled samples from known categories and pseudo-labeled samples from novel categories.
These selected examples are used in the growing phase to expand feature diversity for effective category discovery. Extensive experimental results show that our proposed method consistently shows satisfying performance under multiple practical scenarios compared with existing methods.


%The model is expected to filter out data from the unknown categories, discover novel categories to expand the known set, and maintain classification performance on all the known categories. 

%Therefore, the evaluation of CCD is two-fold: forgetting of the known categories and discovery of the unknown categories.

% 【现有方法在当前框架下的问题】

\begin{figure}[htbp]
  \centering
  \includegraphics[width=0.9\linewidth]{imgs/features.png}
  \caption{Features visualization of model A trained on known categories, model B trained for novel category discovery (based on model A) and the proposed GM model.  }
  \label{fig:features}
\end{figure}





% 【方法设计+实验验证】
%For the compatibility of the two contradicted tasks in CCD, in this paper, we follow the manner of ``divide and conquer'' to propose a framework named \textbf{Split-Merge Network (SMNet)}, which enables us to complete the two tasks in different branches and then merge them together.
% split
%In the split stage of SMNet, we relax the constraints of memorizing previous category to leave full optimization space for category discovery.
%A static-dynamic branch architecture is introduced, where the static branch is frozen for the original category classification, and the dynamic branch is freely updated for category discovery.
%During the discovering process, a static-dynamic distillation loss is also applied to fully utilize existing knowledge for discovering novel categories.
% merge
%In the merge stage of SMNet, we re-tighten the representation for distinguishing both previous and newly-discovered categories with a unified model.
%Exemplar-based classification learning is conducted on all the appeared categories, where Pseudo Label Learning (PLL) is proposed to utilize the discovered categories from the split stage.
%The static and dynamic branches are merged into a single one for the following usage.

% The proposed SMNet contains a static-dynamic branch architecture.
% We firstly derive two branches from the original model, where one is for the original category classification and the another is for mining the novel category.
% To prevent catastrophic forgetting during the incremental process, we introduce prototype and exemplar structure in SMNet and design a static-dynamic distillation loss between branches.
% Specifically, in the split stage, we first utilize an unsupervised representation learning loss to train the dynamic branch and obtain a class-independent representation. Based on feature representation, we divide the input category data into novel categories and known categories to complete novel category discovery. In the merge stage, based on the results of category discovery, we regenerate prototypes and exemplars, and retrain the dynamic branch through the proposed Pseudo Label Learning Loss and merge dynamic branch with the static branch to obtain final model in current incremental process. It is worth noting that we maintain two branches during training, but during inference, we only need to keep the final generated branch.

%The split and merge stages actually achieve the relaxation and tightening on model's representation, respectively, which are found in practice to be essential for the incremental novel category discovery.


%(i) split process with unsupervised representation learning, (ii) merge process with pseudo label representation learning.
%Specifically, in the split process aims both maintaining representations of known categories and discovering novel categories.
% 把branch
%The samples are split into known and novel categories, and the novel samples are clustered led by the unsupervised representation learning.


%The branch is split into a static branch which is frozen for memorizing the classification tasks on the previous categories, and a dynamic branch which is freely optimized for discovering novel categories.
%The novel labels are discovered after the split process and then the merge process fuses the discovered knowledge with the preserved information.
%The discovered categories are merged with known categories by updating the exemplars which are representative samples of each class, and the prototypes representing the categories.
%The pseudo label representation learning (PLL) is applied to generate more compact clusters guided by the discovered label.
%The static/dynamic branches are merged by the exponential moving average strategy into one single branch for inference, while full space is left to guarantee the performance of each branch.

%In experiments, we evaluate methods for CCD under four different settings to cover the application scenarios in the wild. 


%We extend the exemplar set proposed in iCaRL\cite{} to the scheme of unsupervised incremental learning, in which the prototypes represent the discovered novel categories.  
%The construction process of exemplar set is to filter out low-confidence samples based on the geometric property of the unlabeled data.
%Then we introduce pseudo label learning (PLL) to generate more compact clusters guided by the discovered label of exemplars.
%For the multi-branch EMA, we design a two-branch architecture where a \textit{maintaining branch} is stage-wise frozen for memorizing the classification tasks on the previous categories, and a \textit{discovery branch} is freely optimized for discovering novel categories. 
%The teacher-student distillation strategy with EMA is introduced to align the distribution of the two branches for inference, while leave full space to guarantee the performance of each branch.


% 【贡献】问题定义+方法设计+实验
The main contributions of this paper are summarized as follows:
\begin{itemize}
    \item We study a new problem named continuous category discovery, or CCD, which better reflects the challenge of category discovery in the wild. It needs to simultaneously maintain a good performance for known categories and the ability of discovering novel categories.
    %\item We propose a method named SMNet for CCD, where multi-branch EMA is designed to balance the performance between known and novel categories, and prototype-based pseudo label learning is introduced to fully leverage the incremental data for representation learning.
    \item We propose a framework of grow and merge, or GM, for CCD, that is able to resolve the conflicts between the classification task and the task of discovering new categories.
    % , we verify that the feature relaxation and tightening accompanying these two stages are the key to the CCD task.
    \item We conduct experiments under four different settings to fully investigate the scenarios of novel category discovery in the wild. The proposed method shows less forgetting of known categories and better performance for category discovery compared to existing methods.
\end{itemize}

% backup
% With the rapid development of the Internet, huge amounts of data are produced daily. 
% Since it is costly and time-consuming to label entire data, most of these data are unlabeled and waiting to be processed.
% The novel category discovery aims to find the inherent categories from the unlabeled data, by clustering the data from the same class together.
% Although significant improvement on performance is achieved, the recent developed novel category discovery methods only pay attention to the single-stage scenario, in which both labeled and unlabeled data are provided simultaneously.
% In general, these methods learn the representations from all of the labeled and unlabeled data with the semi-supervised technology and cluster the unlabeled data according to the representations.
% However, the data is produced continuously in real world applications.
% In other words, it is impractical to access all of the data at the same time.
% It is necessary to consider the novel category discovery methods under the incremental scheme.
% The incremental data stream is complicated in the real world, which is reflected in categories and labels. A incremental data stream may contain know and unknown categories, meanwhile contain labeled and unlabeled data.
% A practical method should maintain the performance on the known category (or with acceptable forgetting) and discover the novel categories, with the semantic information learned from the labeled data and the latent patterns from the coming incremental data.
% In this paper, we name this problem the incremental novel category discovery, which is derived from practical needs in real world scenarios. There are two main stages in the incremental novel category discovery scheme: the initial pre-training stage and the continuous learning stage.
% During the pre-training stage, the labeled data from a portion of the categories (\ie, the known categories) are provided to initialize the model and the classifier.
% While during the continuous learning stage, the incremental data (\eg, from known categories or novel categories) can be treated as training data.
% The model is required to identify the unlabeled data in the continuous learning stage.
% The main target of the incremental novel category discovery is to keep the performance of the known categories and classify the novel categories all the time.

% Based on the analysis of the related works, we summarize the main challenges of the incremental category discovery scheme:
% \begin{itemize}
%     %\item Catastrophic forgetting. \cite{} %Catastrophic interference in connectionist networks: The sequential learning problem
%     %The learning process of the new data will degrade the performance on the old data. 
%     %Some methods should be applied to overcome the influence of the catastrophic forgetting.
%     %\item Novel category discovery for the unlabeled data. 
%     %For the unlabeled data, the novel category discovery is required to assign clusters to each object.
%     %However, the features may be biased and it is difficult to align the features of the new data with that of the previous data.
%     \item Contradictions between the goals of maintaining the performance on the historical data and discovering the novel categories. 
%     %The empirical experience suggests that in order to keep the information of the old data, the weights of the networks should be kept or change slightly, which limits the networks' capability for novel category discovering.
%     %While in order to discover the novel categories, the feature extractor should be adapted to the novel classes, which affects the quality of the features of the old data.
%     %There exists a trade-off between the performance on the old data and the discovery ability of the new data.
%     \item Feature representation can be improved from the continuous data in the incremental stages while maintaining the performance of the model.
% \end{itemize}

% Existing methods are confronted with different challenges under the scenario of CCD.
% In the field of continuous learning, regularization based methods and replay based methods are used to avoid the catastrophic forgetting. \cite{} % three scenarios
% For example, EWC\cite{} penalize the changes of the network weights according to the importance for previous data.
% LwF\cite{} keeps the performance on the categories seen so far by the techniques from Knowledge Distillation\cite{}. % Distilling the knowledge in a neural network
% iCaRL\cite{} saves representative objects, which is called exemplars, from each category into a limited memory to record the information of the earlier-accessed data.
% These methods keeps the information from previous data during the continuous learning period.
% However, labeled data are required during the continuous learning stage, which constrains the application of these methods in the real world with massive unlabeled data.
% In the field of novel category discovery, cluster based methods are applied to partition the samples from novel categories.
% AutoNovel\cite{} uses ranking statistics to cluster the objects.
% DTC\cite{} transfers the pre-trained embedding to the unlabeled data for the cluster assignments. % Learning to Discover Novel Visual Categories via Deep Transfer Clustering
% These methods discover novel categories by using both labeled and unlabeled data.
% However, these methods do not fit in the continuous learning scheme, as they cannot tackle the challenge of the catastrophic forgetting and the performance on the previous known categories decreases significantly during the continuous learning stage.
% In a word, these recent works are not suitable to the incremental novel category discovery scheme.

% Feature representation can be improved from the continuous data in the incremental stages while maintaining the performance of the model.
% 通过实验发现: 任务是矛盾的, 如何从不断的数据中获益 (cluster head涨)

% The empirical experience suggests that the goals of maintaining the performance on the old data and discovering the novel categories are always contradictory. 
% In order to keep the information of the old data, the weights of the networks should be kept or change slightly, which limits the networks' capability for novel category discovering.
% While in order to discover the novel categories, the feature extractor should be adapted to the novel classes, which affects the quality of the features of the old data.
% Our main goal is to achieve better discovery performance, with the acceptable decrease of the old class performance.

==> NeurIPS 2022 SMNet_0517_arxiv/sections/chap02_problem.tex <==
\section{Problem Definition}

% 2.1 问题定义
% 2.2 抽象流程在问题定义里完成
% 2.3 提出的评价指标
In this section, we formulate the problem of Continuous Category Discovery (CCD).
There are two main stages of the CCD problem, \ie, \textbf{Initial Stage} and \textbf{Continuous Category Discovery Stage}.
The settings of each stage are introduced, together with the evaluation metrics of CCD problem.

\subsection{Setting of Continuous Category Discovery}
During the initial stage, a labeled training dataset $\mathcal{D}^0_{train}= \{ (\bm{x}_i^0, y_i^0)  \}_{i=1}^{N^0}$ is provided to train the model on the initial known category set $\mathcal{C}^0 = \{  1, 2, ..., K^0 \}$, where $\bm{x}_i^0$ is the initial training data, and $y_i^0\in\mathcal{C}^0 $ is the corresponding label.
The model is expected to classify categories in $\mathcal{C}^0$, and learn meaningful representation from the labels' semantic information.

During the continuous category discovery stage, a serial of unlabeled training datasets $\{\mathcal{D}^t_{train}\}_{t=1}^T$ are sequentially provided,
where $\mathcal{D}^t_{train} = \{ \bm{x}_i^t  \}_{i=1}^{N^t}$ indicates the dataset at time $t$.
Though unlabeled, we denote the known or potential appeared categories until time $t$ as $\mathcal{C}^t = \{1, 2, ..., K^t\}$. 
The model is expected to discover newly appeared unknown categories from $\mathcal{D}_{train}^t$, store the representations of the discovered novel categories and maintain the knowledge of the known categories.

% \textbf{Initial Pre-Training Stage}. 
% The teacher encoder $\phi_\mathcal{T}$ is first trained by MoCo \cite{} in a self-supervised scheme.
% Then, the cross entropy loss is applied the train $\phi_\mathcal{T}$ and the classifier.
% The classifier is discarded after the pre-training stage.
% The memory bank containing both exemplars and prototypes are initialized by Eq. \ref{eq:select-exemplars-icarl} and Eq. \ref{eq:mu}.

% \textbf{Continuous Learning Stage}.
% At the beginning of the stage, the student encoder is initialized as the same as the teacher encoder.
% For time $t$, the student encoder and the cluster head are trained by $L_w=L_{TS}+L_{MSE}+L_{BCE}$ for several epochs.
% Then, the samples are sifted by the local geometry property and the memory bank containing the exemplars and prototypes are updated by Eq. \ref{eq:select-exemplars-pseudo}.
% Following the setting that the budget of the memory bank is limited, \cite{} % icarl
% the less important exemplars are discarded.
% After that, $L_{PLL}$ could be applied and $L=L_w+L_{PLL}$ is used to train the model.
% Finally, the student encoder applies EMA with the teacher encoder by Eq. \ref{eq:ema}.

% \textbf{Test}. 
% The features of the test data are first extracted by the student encoder.
% Then, the data is classified and assigned the label $y_i^*$ with the nearest prototype,
% \begin{align}
%     y_i^* = \mathop{\arg\min}\limits_{y=1, \cdots, K^t} || \phi_{\mathcal{S}}^t (x_i^t) - \mu_y  ||.
% \end{align}


\subsection{Evaluation Metrics}

% cluster acc
% forgetting
% discovery
At each time-step $t$, we evaluate the classification performance on the test dataset $\mathcal{D}^t_{test} = \{  (\bm{x}_i^s, y_i^s) | s \leq t     \}$, containing test samples from all the known or previously discovered categories.
For the newly appeared unknown categories, we evaluate the novel category discovery performance.
% The categories $\mathcal{C}^t = \{  1, \cdots, K^t \}$ in which $\mathcal{D}^t_{train}$ is drawn from contain both the already-learned categories $\{  1, \cdots, K^{t-1} \}$ and the novel categories $\{ K^{t-1}+1, \cdots, K^t \}$.
The \textbf{maximum forgetting metric} $\mathcal{M}_f$ and the \textbf{final discovery metric} $\mathcal{M}_d$ are designed for evaluation.
To evaluate the performance of the clustering assignments, we follow the standard practise~\cite{han2021autonovel, drncd} to adopt clustering accuracy on the known categories and the novel categories, denoted as $\text{ACC}_{\text{known}}^t$ and $\text{ACC}_{\text{novel}}^t$, respectively.
The maximum forgetting $\mathcal{M}_f$ is defined as the maximum value of the differences between $\text{ACC}_{\text{known}}^0$ and $\text{ACC}_{\text{known}}^t$ for every $t$ and the final discovery $\mathcal{M}_d$ is defined as the final cluster accuracy on novel categories, \ie, $\mathcal{M}_d = \text{ACC}_{\text{novel}}^T$.
See more details in the supplementary materials.

==> NeurIPS 2022 SMNet_0517_arxiv/sections/chap03_method.tex <==
\section{Method}



\subsection{An Overview of Grow and Merge Framework}
% The CCD problem requires to both maintain the performance on known categories and discover novel categories.
% However, practical experience shows natural contradiction between the two main targets.
% Maintaining classification performance on known categories requires to preserve the learned distribution of representation, while discovering novel categories requires representation shifting for clustering on new data.
The CCD problem requires both maintaining the performance on known categories and discovering novel categories under the continuous learning scheme. For the compatibility of the two tasks, we propose a \textbf{Grow and Merge (GM)} Framework, which is illustrated in Figure \ref{fig:pipeline}.
\par


During the initial stage, the model $\phi^0(\cdot)$ is firstly pre-trained on the initial dataset with labeled data in both supervised and self-supervised manner.
% For samples $x_i^0$ from the $k$-th class with the feature vectors $\phi^0(\mathbf{x}_i^0)$ , we compute the averaged vector $\mu_k$ as the \textit{prototype}.
An \textit{exemplars} set $P_k = \{\mathbf{p}_{k,i}\}$ is constructed as well as the \textit{prototypes}.
The exemplar set contains representative samples for each class while the prototype $\mu_k$ is the averaged feature vector of the exemplars from the $k$-th class.
The exemplar set is constructed
by iteratively picking several typical samples with the principle of maintaining the closest center to the  prototype $\mu_k$, \textit{i.e.} $\mathbf{p}_{k, i} \leftarrow \text{argmin}_{\mathbf{x}} \parallel \mu_k - \frac{1}{i}[\phi^0(\mathbf{x}) + \Sigma_{j=1}^{i-1}\phi^0(\mathbf{p_{k, j}})]\parallel$.
The definitions of prototype and exemplars are adapted from iCaRL \cite{icarl}, which enables us to use a non-parametric classifier that predicts label of a query sample from its nearest prototype's label.


During the continuous category discovery stage,
a dual-branch architecture with a static branch $\phi_S(\cdot)$ and a dynamic branch $\phi_D(\cdot)$ is introduced for training, where both branches are initialized by the pre-trained model $\phi^0(\cdot)$.
At each time-step, GM includes two phases: \textbf{Growing} and \textbf{Merging}. In the growing phase, the novel category data are filtered out from the continuous data and the dynamic branch is trained for novel category discovery.
Then the merging phase fuses the newly discovered and known categories into a single model for unified classification. Knowledge from the frozen static branch is distillated into the dynamic one to avoid forgetting previous classes.

It is noted that though GM maintains two branches during training, only one branch is needed during testing.


\par

Experimental results show significant performance of the GM framework, where the dual-branch architecture and knowledge distillation succeed to balance the feature conflicts between continuous classification and novel categories discovery, and show better performance on both sub-tasks.



\begin{figure}[tbp]
    \centering
    \includegraphics[width=0.9\linewidth]{imgs/pipeline.pdf}
    \caption{\textbf{The proposed Grow and Merge (GM) Framework.}There exist growing and merging phases for each time-step, where a dynamic branch is freely updated for discovering new classes in the growing phase, and then unified with a frozen static branch in the merging phase for maintaining classification on all appeared classes.}
    \label{fig:pipeline}
\end{figure}



\subsection{Growing: Enrich Features with Unlabeled Data}

To achieve novel category discovery from the data stream with both labeled and unlabeled samples from known and unknown classes, we firstly filter out data of unknown classes with \textbf{novelty detection}, and then conduct \textbf{novel category discovery} based on both the new data and the previous model.


\textbf{Novelty Detection} aims to identify the samples belonging to the novel categories in the current training dataset $\mathcal{D}_{train}^t$,
since there may also exist samples from previously known categories.
With the maintained prototypes of known categories, the feature vectors of samples from known categories would lay closer to at least one prototype with a high probability.
Then a novel distance $d_{\text{novel}}$ is defined as the distance between the sample $\mathbf{x}^t_i$ and its nearest prototype, \textit{i.e.} $d_{\text{novel}}(\bm{x}_i^t) = \min_{1 \leq k \leq K^{t}} d(\mu_k, \phi_D^t(\bm{x}_i^t))$, where $d(\cdot, \cdot)$ is the distance function.
Samples with $d_{\text{novel}}$ larger than a threshold $\epsilon$ are filtered out as novel samples for the following process.


\textbf{Novel Categories Discovery and Learning from Static Branch}.
We optimize the dynamic branch $\phi_D^t(\cdot)$ for novel category discovery, guided by both the novel samples and previously learned knowledge for rich feature representation.
(i) For learning and discovering from the novel samples, we adopt an unsupervised representation learning method \cite{han2021autonovel}.
A cluster head $g(\cdot)$ is learned to assign samples $\hat{\bm{x}}_i^t$ to the clusters with novel category indices $\{ K^{t-1}+1, ..., K^t  \}$.
Such an assignment is supervised by the similarity $s_{ij}$ between samples $\hat{\bm{x}}_i^t$ and $\hat{\bm{x}}_j^t$ with a binary cross entropy loss, \textit{i.e.}
\begin{align}
    \mathcal{L}_{\text{BCE}} = -\frac{1}{\hat{N}^t}\sum_{i=1}^{\hat{N}^t}\sum_{j=1}^{\hat{N}^t} \left(  s_{ij} \log {\bm{c}_i^t}^\top \bm{c}_j^t + (1-s_{ij}\log (1- {\bm{c}_i^t}^\top \bm{c}_j^t) ) \right),
\end{align}
where $\hat{N}^t$ is the number of novel category samples at time $t$ (specified or estimated). The similarity $s_{ij}$ is measured by the Winner-Take-All hash (WTA), which equals one when samples share the same top-$k$ channels of their feature vector, otherwise equals zero.



\par

(ii) For learning from the static branch $\phi_D^t(\cdot)$ with previously learned knowledge, we introduce a \textit{static-dynamic distillation loss} to transfer the representation learned from labeled data in the static branch into the dynamic one:
\begin{align}
    \label{eq:ts}
    \mathcal{L}_{\text{SD}} =  \frac{1}{N^t}\sum_{i}^{N_t}d\left( \bm{z}_i^t  , \bm{z}\prime_i^t \right)=  \frac{1}{N^t}\sum_{i}^{N_t}d\left( \phi_S(\bm{x}_i^t ) , \phi_D^t(\bm{x}_i^t ) \right)
\end{align}
The joint loss $\mathcal{L}_{\text{BCE}}$ and $\mathcal{L}_{\text{SD}}$ enables the dynamic branch to discovering novel categories with richer feature representation, and the cluster head $g(\cdot)$ could assign new labels to the novel category data $\hat{\bm{x}}_i^t$.


\subsection{Merging: Unification of Categories and Branches}

After the Growing phase, both categories and models contain two parts for the known and novel categories, respectively. The Merging phase reunifies them together for all the appeared categories.

\subsubsection{Category Unification: Continuous Learning for Newly Discovered Categories}

To merge the novel categories discovered in Growing phase into the classifier,
we firstly \textbf{sift samples} to construct the exemplar sets of the novel categories, then refine the model representation using a \textbf{pseudo label representation learning} for classification on both known and novel classes.

\textbf{Sample Sifting} aims to filter out incorrectly-assigned samples based on their cluster confidence.
The assigned class indices by $g(\cdot)$ are denoted as the pseudo-labels of the novel samples, which may inevitably have errors and lead to less reliable prototypes of the novel categories.
We sift out these potentially noisy samples via the local sample density, with the assumption that samples from the same class would lay tightly.
Suppose $\mathcal{N}_j(\hat{\bm{z}}_i^t)$ indicates the $j$ nearest neighbors of $\hat{\bm{z}}_i^t$ from the same class.
The local sample density $G_j(\hat{\bm{z}}_i^t)$ is defined as the distance between $\hat{\bm{z}}_i^t$ and its $j$-th nearest neighbors, \textit{i.e.} $G_j(\hat{\bm{z}}_i^t) = \max_{\bm{z}\in \mathcal{N}_j(\hat{\bm{z}}_i^t)} d(\hat{\bm{z}}_i^t, \bm{z})$.
Samples with larger $G_j$ are sifted out, then the left samples are denoted as $\Tilde{\bm{x}}_i^t$ with pseudo labels $\Tilde{c}_i^t$.



\textbf{Pseudo Label Representation Learning.}
Based on the sifted novel samples of the $k$-th novel category, we firstly construct the exemplar set $P_k = \{\mathbf{p}_{k,i}\}$. Without knowing the prototype $\mu_k$, \textit{i.e.} the explicit center of the $k$-th category, we estimate it with the averaged vectors of sifted samples.
For the purpose of continuous classification on all appeared classes, it is required to tighten the sparse representation distribution learned in the growing phase.
Pseudo Label Learning (PLL) loss is introduced here.
Compared with commonly-used Cross Entropy loss, PLL does not require an explicit classifier and thus does not modify the deployed model structure during the continuous phase.
The loss function $\mathcal{L}_{\text{PLL}}$ aims to pull exemplars pull the exemplars $\bm{p}_k$ and the corresponding prototypes $\mu_k$ closer, and push $\bm{p}_k$ away from the other prototypes $\mu_j (j\neq k)$:
\begin{align}
    \mathcal{L}_{\text{PLL}} = - \frac{1}{K^t}\sum_{k=1}^{K^t} \frac1{|P_k|}\sum_{i=1}^{|P_k|} \log \frac{\exp (\phi_D^t(\bm{p}_{k,i})\cdot \mu_k / \tau)}{\sum_{j=1}^{K^t} \exp (\phi_D^t(\bm{p}_{k,i})\cdot \mu_j / \tau)},
\end{align}
where $\tau$ is a temperature hyper-parameter.
To avoid catastrophic forgetting, based on data in the latest exemplars, the static-dynamic distillation loss in Eq. \ref{eq:ts} is also employed here.

\subsubsection{Branch Unification: Merging Multiple Branches into One Unified Model}

During the above process, the dynamic branch is optimized to classify all appeared categories.
In order to reduce computation cost and further utilize the representation of the static branch trained from labeled data, we merge the two branches into a single one.  In experiments, we found such a branch merging can further improve the recognition performance. To fuse the representation of $\phi_S$ and $\phi_D^t$, the exponential moving average strategy (EMA) is applied:
\begin{align}
    \label{eq:ema}
    \theta_{\phi_D^t}\longleftarrow \alpha \theta_{\phi_S} + (1-\alpha) \theta_{\phi_D^t},
\end{align}
where $\alpha$ is the momentum hyper-parameter to control the weight of fusion, generally valued close to 1 ($\alpha = 0.99$ in this paper).


\subsection{Estimating the Number of Novel Categories}
Grow and Merge framework is proposed to solve the CCD problem.
GM is a generic framework which focuses on how to implementing continuous classfication and novel classes discovery at the same time.
Estimating the number of novel categories has been studied in literatures including \cite{han2020automatically,drncd}, which can be easily employed in GMNet.
For each time step $t$, the representations of the coming data $\phi(\mathbf{x}^t)$ is mixed together with the exemplars $P$.
The semi-Kmeans algorithm  is applied on these mixed data with different number of clusters, and the cluster accuracy on the exemplars are evaluated based on the pseudo labels of the exemplars.
The number of the clusters with the highest cluster accuracy is estimated as the number of novel categories.


==> NeurIPS 2022 SMNet_0517_arxiv/sections/chap04_experiments.tex <==
\section{Experiments}
\label{sec:exp}
% 1.	settings (70/10/10/10, ……)
% 2.	implementation details
% 3.	results
%   a)	ours, upper bound, autonovel
%   b)	pll, ce, ssl的影响
%   c)	multi-branch, 不同深度，new branch的不同初始化方式
%   d)	teacher-student，不同方式
%   e)	ema，ema参数，ema方式
%   f)	复杂情况的结果

In this section, we design experiments in different scenarios to simulate the varying cases of real-world applications, which enables us to fully investigate the performance and flexibility of the proposed method.
Two main evaluation metrics, namely, maximum forgetting $\mathcal{M}_f$ and final discovery $\mathcal{M}_d$ are employed to measure the performance.
CIFAR-100~\cite{cifar},  CUB-200~\cite{cub200} and ImageNet-100~\cite{imagenet, imagenet100} representing the small, middle and large scale datasets are used in the experiments.

\textbf{Experimental Scenarios}.We formulate four different scenarios for experiments as follows.
(1) \textit{Class Incremental Scenario (CI)}:
the data are only drawn from novel categories.
(2) \textit{Data Incremental Scenario (DI)}:
the data are only drawn from the known categories.
(3) \textit{Mixed Incremental Scenario (MI)}: the data are drawn from both novel and known categories.
(4) \textit{Semi-supervised Mixed Incremental Scenario (SMI)}:
the data are drawn from both novel and known categories, and a portion of the data are labeled,
which is closed to the real-world application.

\input{tables/tab_scenarios}

The settings of these scenarios are summarized in Table~\ref{tab:scenario}.
We mainly focus on the standard scenario CI in this paper, while the experimental results on DI, MI, and SMI are reported to demonstrate the flexibility of the proposed method.
Each scenario contains $T=3$ time-steps of the continuous learning stage.
Details of the scenarios could be found in supplementary materials.
% \begin{itemize}
% \item \textit{Class Incremental Scenario (CI)}, where the newly appeared data are only drawn from the novel categories, \ie, $\mathcal{C}^t \cap ( \mathcal{C}^{t-1} \cup \cdots \cup \mathcal{C}^0  )=\emptyset, \forall t\in\{ 1, \cdots, T  \}$.
% CI is a standard scenario that only requires the models to learn from the novel samples and keep the performance of the known categories.
% \item \textit{Data Incremental Scenario (DI)}, where data are only drawn from the known categories, \ie, $\mathcal{C}^0= \mathcal{C}^t, \forall t\in \{1, \cdots, T\}$.
% DI is a simple scenario, which evaluates the models' capability to improve the feature representation with the continuous unlabeled data.
% \item \textit{Mixed Incremental Scenario (MI)}, where data are drawn from both novel categories and the known categories, \ie, $\mathcal{C}^0\subset \mathcal{C}^1 \subset \cdots \subset \mathcal{C}^T$.
% MI is more complicated than CI, where models are further required to identify whether the data comes from novel categories or not.
% \item \textit{Semi-supervised Mixed Incremental Scenario (SMI)}, where data are drawn from both novel categories and the known categories, \ie, $\mathcal{C}^0\subset \mathcal{C}^1 \subset \cdots \subset \mathcal{C}^T$, and a portion of the data are labeled.
% SMI is closer to the real-world application, where both labeled and unlabeled samples are provided in the incremental stages.
% \end{itemize}



% 这里刚介绍完四种就说主要做第一种是不是不太好？

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}


% \textbf{Scenarios Details}.
% % For all of the scenarios, the total time-steps $T$ is set to 3.
% For CI, 70\%/10\%/10\%/10\% classes of the CIFAR-100~\cite{cifar},  CUB-200~\cite{cub200} and ImageNet-100~\cite{imagenet, imagenet100} datasets are used in the initial pre-training stage and the following 3 time-steps of the continuous learning stage, respectively.
% For DI, 25\% of the data are used for the initial pre-training stage, and 75\% are used for the continuous learning stage, with 25\% data at each time-step.
% For MI, 87\% data from 0-70 classes in CIFAR-100 are used for initial pre-training stage.
% 7\% of data from 0-70 classes, 70\% data from 70-80 classes are used for $t=1$ during the continuous learning stage.
% 2\% data from 0-70 classes, 20\% data from 70-80 classes and 90\% data from 80-90 classes are used for $t=2$.
% 3\% data form 0-70 classes, 10\% data from 70-80 classes, 10\% data from 80-90 classes and all of the data from 90-100 classes are used during $t=3$.
% For SMI, 20\% of the data from MI are labeled during $t=1,2,3$.
%可能要改成详细情况我们在补充材料里说明

% MLP config之类的也放附录
\textbf{Implementation Details}.
For all experiments, we train the model 100 epochs using $\mathcal{L}_{\text{BCE}}+\mathcal{L}_{\text{SD}}$ loss and 100 epochs using $\mathcal{L}_{\text{BCE}}+\mathcal{L}_{\text{SD}}+\mathcal{L}_{\text{PLL}}$ loss for each time-step $t$.
The $\alpha$ for EMA is set to 0.99.
The novelty detection threshold $\epsilon$ is set to 0.6.
15 neighbors are selected for each sample during sample sifting and the top 50\% samples with larger local density are sifted out.
The temperature $\tau$ used in $\mathcal{L}_{\text{PLL}}$ is set to 0.1. Mean Squared Error (MSE) Consistency Loss
$\mathcal{L}_\text{MSE} = \frac1{N^t}\sum_i^{N^t} || \phi_D^t (\bm{x}_i^t) - \phi_D^t (\bm{x}\prime_i^t)  ||_2^2$
is also used during the continuous learning following AutoNovel~\cite{han2021autonovel}, where $\bm{x}\prime_i^t$ denotes the augmentation of $\bm{x}_i^t$.
More details could be found in supplementary materials.
% Besides, the MSE loss is applied on the features of different augmentations during the continuous learning stage,
% \begin{align}
%     \mathcal{L}_{\text{MSE}} = \frac1{N^t}\sum_i^{N^t} || \phi_D^t (\bm{x}_i^t) - \phi_D^t (\bm{x}'_i^t)  ||_2^2,
% \end{align}
% where $\bm{x}'_i^t$ denotes the augmentation of $\bm{x}_i^t$.

\subsection{Comparisons with SOTA methods on CI scenario}

We first investigate the performance of the proposed method under CI scenario.
CIFAR-100, CUB-200, ImageNet-100, Stanford-Cars, FGVC-Aircraft, and ImageNet-200 are used in this experiment.
The maximum forgetting $\mathcal{M}_f$ and final discovery $\mathcal{M}_d$ are reported in Table~\ref{tab:ci}.
Since there are few works about continuous novel category discovery and recent works about incremental learning may not fit the unsupervised scenario, we compare the proposed method with the lower bound of $\mathcal{M}_f$ and the upper bound of $\mathcal{M}_d$, two recent methods for novel category discovery, \ie, AutoNovel~\cite{han2021autonovel}
and DRNCD~\cite{drncd}, %\cite
and the combinations of the novel category discovery methods and continuous learning methods.

%We apply the origin AutoNovel~\cite{han2021autonovel} method with offline setting as the upper bound of $\mathcal{M}_d$ in this scenario and K-Means~\cite{kmeans} as the lower bound of $\mathcal{M}_f$.
It is noticed that there is not an exact lower/upper bound method under the CI scenario.
Therefore, we conduct two methods under the \textbf{offline setting}, where all of the data containing both known and novel categories are available in a single stage.
We present the results of K-means~\cite{kmeans} as a reference to the lower bound of $\mathcal{M}_f$, and the original AutoNovel method as the upper bound of $\mathcal{M}_d$.
% As there exists trade-off between $\mathcal{M}_f$ and $\mathcal{M}_d$,
It should be enhanced that the lower/upper bound results are for reference and could not exactly represents the best performance on both $\mathcal{M}_f$ and $\mathcal{M}_d$.
Since recent novel category discovery and incremental learning methods usually contain multiple stages, we chose AutoNovel and LwF \cite{lwf} and combine them for comparison based on the flexibility of implementation.
It is observed that AutoNovel with LwF greatly improves the $\mathcal{M}_f$ and $\mathcal{M}_f$ compared to the online version of AutoNovel. However, such a simple combination not completely solves the feature conflict caused by the two different tasks.
The proposed GM framework divides and conquers the conflict of features and achieves the best results among the compared methods (that conduct classification and discovery training in one single phase) on all datasets, indicating the effectiveness of the two phases of growing and merging.
% On CIFAR-100, GM decreases the $\mathcal{M}_f$ for 85\%, 84\%, 65\% and 72\% compared with AutoNovel, DRNCD, AutoNovel + LwF and iCaRL(fixed exemplars) + LwF, and obtains $\mathcal{M}_d$ gain of 46\%, 218\% and 26\% compared with AutoNovel, DRNCD and AutoNovel + LwF, respectively.
% On CUB-200, GM decreases $\mathcal{M}_f$ for 57\% and 56\% compared with DRNCD and iCaRL(fixed exemplars) + LwF, and increases $\mathcal{M}_d$ for 37\% and 19\% compared with AutoNovel and AutoNovel + LwF, respectively.
% GM even outperforms $\mathcal{M}_d$ of the offline AutoNovel on the CUB-200 dataset, which learns from all of the data in a single stage.
% On ImageNet-100 dataset, the proposed method decreases $\mathcal{M}_f$ for 19.8\% compared with iCaRL (fixed exemplars) + LwF, and increases $\mathcal{M}_d$ 238\%, 310\% and 253\% compared with AutoNovel, DRNCD and AutoNovel + LwF, respectively.
% There are two main reasons that our method outperforms these baseline methods.
% First, as our method maintains the origin representations of the known categories while AutoNovel and DRNCD corrupts the representations during the continuous learning stage, the maximum forgetting of our method is much lower than the baseline methods.
% Second, our method improve the representation by the sifting strategy and pseudo label learning with the unlabeled data, while the other methods could not benefit from the continuous unsupervised learning.

\input{tables/tab_ci}

\begin{minipage}{\textwidth}
    \begin{minipage}[t]{0.3\textwidth}
        \centering
        \makeatletter\def\@captype{table}\makeatother\caption{Experimental results under DI scenario. (mean$\pm$std.)}
        \renewcommand\arraystretch{1.03}
        \resizebox{\textwidth}{!}{%
            \begin{tabular}{@{}lr@{}}
                \toprule
                Method                                            & $\mathcal{M}_f$ $\downarrow$ \\ \midrule
                Original Model                                    & 0                            \\
                % KMeans~\cite{kmeans} & 13.83 \\
                Pseudo iCaRL                                      & 9.51$\pm$0.35                \\
                DeepClustering~\cite{deepclustering}              & 1.61$\pm$0.44                \\
                AutoNovel$^*$~\cite{wta, DBLP:conf/iccv/JiaHZG21} & 0.30$\pm$0.07                \\
                GM                                                & \textbf{-23.68$\pm$0.27}     \\ \bottomrule
            \end{tabular}
        }
        \label{tab:di}
    \end{minipage}
    \hspace{0.3cm}
    \begin{minipage}[t]{0.67\textwidth}
        \centering
        \makeatletter\def\@captype{table}\makeatother\caption{Experimental results under MI and SMI scenario. (mean$\pm$std.)}
        \resizebox{\textwidth}{!}{%
            \begin{tabular}{@{}lrrrr@{}}
                \toprule
                                                             & \multicolumn{2}{c}{\textbf{MI}}                   & \multicolumn{2}{c}{\textbf{SMI}}                                                                                                                    \\
                Method                                       & \multicolumn{1}{l}{$\mathcal{M}_f$ $\downarrow$ } & \multicolumn{1}{l}{$\mathcal{M}_d$ $\uparrow$} & \multicolumn{1}{l}{$\mathcal{M}_f$ $\downarrow$ } & \multicolumn{1}{l}{$\mathcal{M}_d$ $\uparrow$} \\ \midrule
                AutoNovel~\cite{han2021autonovel}            & 63.25$\pm$0.19                                    & 5.74$\pm$0.17                                  & 60.98$\pm$1.27                                    & 21.61$\pm$3.94                                 \\
                DRNCD~\cite{drncd}                           & 43.81$\pm$1.71                                    & 5.12$\pm$0.98                                  & 56.27$\pm$1.13                                    & {47.67$\pm$1.66}                               \\
                AutoNovel + LwF~\cite{han2021autonovel, lwf} & 61.89$\pm$0.87                                    & 5.59$\pm$1.99                                  & 61.45$\pm$2.43                                    & 31.84$\pm$1.06                                 \\
                DRNCD + LwF~\cite{drncd, lwf}                & 35.44$\pm$4.61                                    & 4.10$\pm$0.99                                  & 62.38$\pm$1.01                                    & \textbf{52.53$\pm$1.92}                        \\
                GM w/o. novelty detection                    & \textbf{ 4.74$\pm$0.78}                           & 10.61$\pm$3.37                                 & \textbf{8.43$\pm$0.45}                            & 31.42$\pm$0.76                                 \\
                GM                                           & 9.65$\pm$0.32                                     & \textbf{30.58$\pm$1.13}                        & 9.41$\pm$0.31                                     & 35.52$\pm$1.21                                 \\ \bottomrule
            \end{tabular}
        }
        \label{tab:mi-smi}
    \end{minipage}
\end{minipage}

\subsection{Extended Experiments on More Complicated Scenarios}
In this part, we extend GM to more complicated scenarios: DI, MI, and SMI scenarios. Experiments are conducted on CIFAR-100 and the results are listed in Table~\ref{tab:di} and Table~\ref{tab:mi-smi}. Due to there is no novel category in the incremental unlabeled data under DI, we remove the cluster head in the AutoNovel to form compared method $\text{AutoNovel}^{*}$. Incremental learning method iCaRL~\cite{icarl} combined with pseudo label assignment and unsupervised learning method DeepClustering combined with finetuning on incremental data are also chosen for comparisons. As shown in Table~\ref{tab:di}, after finetuning on the incremental unlabeled data, all comparison methods show the catastrophic forgetting effect, and the performances are even worse than the original model. GM avoids catastrophic forgetting and effectively utilizes continuous unlabeled data, further improving the final performance. In MI and SMI scenarios, incremental data are mixed with known and novel categories, which makes label assignment for incremental data more difficult. Nonetheless, as shown in Table~\ref{tab:mi-smi}, GM can still effectively avoid catastrophic forgetting and achieve superior performance (especially on $\mathcal{M}_f$) with the help of two phases of growing and merging, compared to the comparison methods.

\subsection{Estimating the Number of Novel Categories}
In this part, experiments with the unknown number of novel categories are conducted on CIFAR-100 and ImageNet-100 in CI, MI, and SMI scenario.
The model should estimate the number of novel categories, discover the novel categories, and maintain the performance on the known categories during each time step.
The experimental results are provided in Table~\ref{tab:est}.
It could be found that GM without knowing the ground-truth number of novelty classes can still outperform other methods using the ground-truth number of novelty classes.
GM model only has 1.33 and 2.47 decreases under CI scenario, and no more than 4.71 decreases under more challenging MI and SMI scenarios, which is acceptable.

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{graphicx}
\begin{table}[]
    \centering
    \caption{Estimation of the number of novel class in each time step, as well as the corresponding performances using the estimated number.}
    \label{tab:est}
    \resizebox{\textwidth}{!}{%
        \begin{tabular}{@{}llll|ll@{}}
            \toprule
                              & \#Classes ($t=2$) & \#Classes  ($t=3$) & \#Classes  ($t=4$) & $\mathcal{M}_f$ & $\mathcal{M}_d$ \\ \midrule
            CIFAR-100 (CI)    & 11                & 13                 & 13                 & 9.91$\pm$0.32   & 34.41$\pm$0.96  \\
            ImageNet-100 (CI) & 12                & 13                 & 13                 & 9.19$\pm$0.51   & 26.26$\pm$1.27  \\
            CIFAR-100 (MI)    & 14                & 13                 & 13                 & 0.33$\pm$0.59   & 28.06$\pm$0.43  \\
            CIFAR-100 (SMI)   & 14                & 14                 & 14                 & 9.63$\pm$0.38   & 35.31$\pm$1.60  \\ \bottomrule
        \end{tabular}%
    }
\end{table}

% We list the experimental results of the three scenarios in Table~\ref{tab:di} and Table~\ref{tab:mi-smi}.
% The experiments under DI scenario are conducted on the CIFAR-100 dataset and are shown in Tabel~\ref{tab:di}.
% As there is few work for incremental clustering, some methods for clustering or incremental learning are adapted for this scenario.
% K-Means~\cite{kmeans} clusters the samples based on the representation pre-trained on the known categories.
% Pseudo iCaRL uses pseudo label provided by iCaRL~\cite{icarl}
% itself to train the representation, rather than the ground truth label.
% Deepclustering~\cite{deepclustering}
% extracts the feature by resnet, assign pseudo labels by K-Means algorithm and train the classifier with the pseudo labels.
% Ft-$\mathcal{L}_{\text{BCE}}$ finetunes the pre-trained feature extractor using $\mathcal{L}_{\text{BCE}}$ with WTA~\cite{wta,DBLP:conf/iccv/JiaHZG21} for clustering.

% Experimental results show that our method significantly outperforms the other four methods.
% The negative value of $\mathcal{M}_f$ demonstrates that the feature representation can be improved from the continuous data in the incremental stages.
% This ability comes from the pseudo label learning, which pulls the exemplars and the corresponding prototypes closer, and pushes the exemplars and the prototypes of different classes away.

% \begin{table}[]
% \centering
% \caption{Experimental results under DI scenario}
% \begin{tabular}{@{}lr@{}}
% \toprule
%               & $\mathcal{M}_f$ $\downarrow$  \\ \midrule
% ResNet + K-Means & 13.83 \\
% Pseudo iCaRL   & 9.90        \\
% Deepclustering & 2.10        \\
% Finetune ($\mathcal{L}_{\text{BCE}}$ with WTA) & 0.38 \\
% GM           & \textbf{-23.87}     \\ \bottomrule
% \end{tabular}
% \label{tab:di}
% \end{table}


% \begin{table}[]
% \centering
% \caption{Experimental results under DI, MI and SMI scenario}
% \begin{tabular}{@{}lrlrrrr@{}}
% \toprule
%  & \multicolumn{1}{c}{\textbf{DI}} & & \multicolumn{2}{c}{\textbf{MI}} & \multicolumn{2}{c}{\textbf{SMI}}  \\
%   & \multicolumn{1}{l}{$\mathcal{M}_f$ $\downarrow$ } &             & \multicolumn{1}{l}{$\mathcal{M}_f$ $\downarrow$ }  & \multicolumn{1}{l}{$\mathcal{M}_d$ $\uparrow$} & \multicolumn{1}{l}{$\mathcal{M}_f$ $\downarrow$ }  & \multicolumn{1}{l}{$\mathcal{M}_d$ $\uparrow$} \\ \midrule
% ResNet + K-Means\cite{kmeans} & 13.83 & AutoNovel\cite{han2021autonovel}      & 63.11                          & 5.92       & 62.44 & 17.33                   \\
% Pseudo iCaRL   & 9.90 & DRNCD\cite{drncd} & 44.79                          & 4.00   & 55.84 & \textbf{47.07}                      \\
% Deepclustering\cite{deepclustering} & 2.10 & AutoNovel + LwF\cite{han2021autonovel, lwf} & 62.51 & 3.34 & 64.25 & 30.87 \\
% Finetune ($\mathcal{L}_{\text{BCE}}$)\cite{wta, DBLP:conf/iccv/JiaHZG21} & 0.38 & GM w/o. OOD detection &       \textbf{ 4.56} &     8.53      & \textbf{8.07} & 30.93       \\
% GM           & \textbf{-23.87} & GM           & 9.83                           & \textbf{32.41}     & 8.84 & 37.23                     \\ \bottomrule
% \end{tabular}
% \label{tab:di-mi-smi}
% \end{table}









% \subsection{Performance under MI scenario}

% The experiments under MI scenario are conducted on the CIFAR-100 dataset, shown in Tabel~\ref{tab:mi-smi}.
% We select AutoNovel~\cite{han2021autonovel}, DRNCD~\cite{drncd}, AutoNovel + LwF~\cite{han2021autonovel, lwf} for comparison.
% The results of GM without OOD detection are also reported.
% GM decreases $\mathcal{M}_f$ for 78\% compared with DRNCD and achieves gain of 447\% compared with AutoNovel.
% Compared with CI scenario, MI is more complicated, as $\mathcal{D}_{train}^t$ in MI contains both known and novel categories while that in CI only contains novel categories.
% The models should identify the known and novel categories in MI.
% In the experimental results, our method shows a superior performance improvement over the compared methods in this difficult scenario:
% $\mathcal{M}_f$ increases for 0.4\% and $\mathcal{M}_d$ decreases for 9.4\%, which is still acceptable.
% The adaptability of GM comes from the OOD detection procedure, which %ignores the known category samples to avoid affecting the novel category discovery.
% aims to identify the samples belong to the novel categories in order to reduce the impact of the known category samples and un-confident samples during discovering.
% %We also conduct experiments on the model without OOD detection.
% %OOD detection aims to identify the samples belong to the novel categories in order to reduce the impact of the known category samples and un-confident samples during discovering.
% The model without OOD detection performs better on $\mathcal{M}_f$, however, decreases $\mathcal{M}_d$ for 74\%, which is not acceptable in real-world applications.

% \subsection{Performance under SMI scenario}

% The experiments under SMI scenario are conducted on the CIFAR-100 dataset, shown in Tabel~\ref{tab:mi-smi}.
% SMI is more realistic than MI, as the continuous coming data in SMI contains both labeled and unlabeled samples.
% The models could benefit from the semantics information of the labeled data.
% However, the complex data combination brings difficulty to design the model.
% The results show that all of the methods perform better than that under MI scenario.
% However, GM still outperforms these compared method with the consideration of both $\mathcal{M}_f$ and $\mathcal{M}_d$.
% GM decreases $\mathcal{M}_f$ for $\sim$85\% and increases $\mathcal{M}_d$ for 114\% and 20.6\% compared with AutoNovel and AutoNovel + LwF, respectively.
% Although DRNCD performs better on $\mathcal{M}_d$ for discovery compared with GM, DRNCD still has the maximum forgetting $\mathcal{M}_f$ for 55.84\%, almost 6 times as ours, which is not practical in real world application.
% Again, experiments on the model without OOD detection is conducted.
% The model without OOD detection decreases $\mathcal{M}_f$ for 8.7\% and $\mathcal{M}_d$ for 17\%.
% The impact of the removal of OOD detection reduces compared with the MI scenario, as the labeled data provides more semantic information during the continuous learning stage.
% With the consideration of both $\mathcal{M}_f$ and $\mathcal{M}_d$, GM still outperforms the model without OOD detection.


\begin{figure}[t]
    \centering
    \subfigure[]{
        \begin{minipage}{0.48\textwidth}
            \centering
            \includegraphics[width=1\textwidth]{imgs/dist_.png}
        \end{minipage}
    }
    \subfigure[]{
        \begin{minipage}{0.48\textwidth}
            \centering
            \includegraphics[width=1.\textwidth]{imgs/features_2.png}
        \end{minipage}
    }
    \centering
    \caption{(a) The intra-/inter- class distance measured throughout the growing and merging phases. (b) Feature visualizations at different time of GM, where the colored dots denote previously appeared classes, and the gray dots denote the newly appeared classes without labels.}
    \label{fig:dist-feature}
\end{figure}

\subsection{Ablation Studies}

% Oringal
% Previous experimental results indicate Grow and Merge framework can better accomplish the continuous learning and the novel category discovery in multiple scenarios. Here we provide intra- and inter- class distance among features and the visualizations in different time of GM in Figure~\ref{fig:dist-feature}. It can be clearly observed that with the alternation of the growing and merging phases, the intra-class distance first increases and then decreases. The classes are relatively compact but overlapped with others before growing phase, loose after growing phase, and compact and separated with others after merging phase. The results are consistent to our motivation that the GM relaxes and tightens the features alternatively to resolve the feature conflicts caused by CCD task.
% \par
% We also provide detailed analysis for all proposed key components of GM. Ablation studies are conducted on the CIFAR-100 dataset under CI scenario, shown in Table~\ref{tab:abla:1} and Tabel~\ref{tab:abla:2}.


Previous experimental results indicate Grow and Merge framework can better accomplish the continuous learning and the novel category discovery in multiple scenarios. Here we provide intra- and inter- class distance among features and the visualizations in different time of GM in Figure~\ref{fig:dist-feature}. It can be clearly observed that with the alternation of the growing and merging phases, the intra-class distance first increases and then decreases. The classes are relatively compact but overlapped with others before growing phase, loose after growing phase, and compact and separated with others after merging phase. The results are consistent to our motivation that the GM relaxes and tightens the features alternatively to resolve the feature conflicts caused by CCD task.
The detailed analysis for all proposed key components of GM are provided. Ablation studies are conducted on the CIFAR-100 dataset under CI scenario, shown in Table~\ref{tab:abla:1} and Tabel~\ref{tab:abla:2}.
We also provide the experiments about estimating the number of novel categories in the supplementary material.




% \textbf{Maintaining}. Maintaining aims to retain the performance of known classes when the model discovers novel categories during the split stage by introducing the cross entropy loss (CE). It can be observed that the preserving the representation of known classes degrades the performance on $\mathcal{M}_d$, which validates that relaxing the constraint of memorizing previous category information can facilitate category discovery.

% \textbf{PLL}.
% PLL aims to improve the representation, which pulls the exemplars and the corresponding prototypes closer, and pushes the exemplars and the prototypes of different classes farther.
% Except PLL, we evaluate the performance of the models replacing PLL with other representation learning methods.
% \textit{CE} represents cross entropy loss which is employed on the cluster assignments and the pseudo label given by the prototypes.
% \textit{SSL} denotes standard InfoNCE loss~\cite{simclr,moco} which is applied among the samples and the augmentations to learn the representation.
% The experimental results show that the model with CE performs better on the known categories but worse on discovering novel categories.
% The model with CE + PLL performs between CE and PLL.
% Similarly, SSL also performs better on known categories and worse on novel categories.
% Therefore, we find that both CE and SSL could be alternative or combined with PLL, with the consideration of the importance of known category maintaining and novel category discovery.

% \textbf{Multi-Branch}.
% The multi-branch aims to maintain known category information and discover novel categories on different branch.
% We evaluate the performance of the model with a single branch.
% The results show that $\mathcal{M}_d$ is affected slightly but $\mathcal{M}_f$ increases significantly, which demonstrates the importance of the multi-branch to preserve already learned representations.
% Besides, the initialization of $\phi_D^0$ also matters, which makes both $\mathcal{M}_f$ and $\mathcal{M}_d$ worse.

% \textbf{Static-Dynamic Mechanism}.
% We proposed $\mathcal{L}_{\text{SD}}$ to align the feature space of the static branch $\phi_S$ and the dynamic branch $\phi_D^t$.
% The performances of the model without $\mathcal{L}_{\text{SD}}$ and the model replacing $\mathcal{L}_{\text{SD}}$ with DINO~\cite{DBLP:conf/iccv/CaronTMJMBJ21} are presented.
% DINO is an alternative of $\mathcal{L}_{\text{SD}}$ which considers the features of the branches after Softmax as the probability distributions and applies the distill loss %cite
% to make the distributions similar.
% The results show that the model without $\mathcal{L}_{\text{SD}}$ performs worse on both $\mathcal{M}_f$ and $\mathcal{M}_d$.
% This comes from the reason that the separation of the feature spaces leads to the failure of the prototype mechanism.
% Compared with the model with $\mathcal{L}_{\text{SD}}$, the model with DINO increases $\mathcal{M}_f$ for 3\% and decreases $\mathcal{M}_d$ for 6.3\%.
% Therefore, $\mathcal{L}_{\text{SD}}$ is used in this paper.

% \textbf{Sifting}.
% Sifting aims to sift out samples with low cluster confidence.
% Except the criterion based on the local geometry property, there are several potential criteria to sift samples.
% \textit{CP} select the portion of all samples with the highest confidence score given by the cluster head.
% \textit{CPC} select the portion of samples from each class with the highest confidence score.
% \textit{CT} select the samples with the confidence score higher than a given threshold.
% The results show that 1) for $\mathcal{M}_f$ the model without sifting and CP performs worse, and CPC, CT and the local geometry property based method performs at almost same level; 2) for $\mathcal{M}_d$, the local geometry property based method outperforms all of these compared methods.
% Therefore, the local geometry property based method is used in this paper.


% \textbf{EMA}.
% EMA aims to fuse the information of $\phi_S$ and $\phi_D^t$.
% We evaluate the performance of the model without EMA.
% $\mathcal{M}_f$ increases for 55\% and $\mathcal{M}_d$ decreases for 14\%, which demonstrates the necessity of EMA.
% We also consider an alternative fuse method which assigns $\phi_S\leftarrow \phi_D^t$ after the update of $\phi_D^t$ by Eq.~\ref{eq:ema}.
% $\mathcal{M}_d$ is significantly affected, with the decrease of 33\%.
% Therefore, we use the fixed $\phi_S$ in this paper.


\textbf{Growing Phase}.
We investigate the performance of introducing additional methods for representation learning in the growing phase.
Combining with cross entropy loss (CE) of the exemplars degrades $\mathcal{M}_d$,
%It can be observed that the preserving the representation of known classes degrades the performance on $\mathcal{M}_d$,
which validates that relaxing the constraint of memorizing previous category information can facilitate category discovery.
Thus, we further introduce more relaxed self-supervised methods.
Combing SimCLR \cite{simclr} also degrades $\mathcal{M}_d$, which could be attributed that pushing the representation of negative samples away hurts the performance.
An alternative method SimSiam \cite{simsiam} achieves comparable performance without pushing negative samples, which also validates the importance of a relaxed representation in this phase.

\textbf{Merging Phase}.
In the merge phase, PLL is employed to improve the representation.
We evaluate the performance of the models replacing PLL with other representation learning methods.
\textit{CE} represents cross entropy loss with the pseudo label given by the prototypes and \textit{SSL} denotes standard InfoNCE loss~\cite{simclr,moco}.
%The experimental results show that the model with CE performs better on the known categories but worse on discovering novel categories.
%The model with CE + PLL performs between CE and PLL.
%Similarly, SSL also performs better on known categories and worse on novel categories.
The experimental results demonstrate that, though these alternative methods could perform competitively on known classes, they sacrifice the performance of discovering novel classes.
% CE and SSL could be alternative or combined with PLL, with the consideration of the importance of known category maintaining and novel category discovery.




% \begin{figure}[tbp]
%   \centering
%   \includegraphics[width=0.9\linewidth]{imgs/dist_.png}
%   \caption{The intra- and inter- class distance of different time of GM Framework.}
%   \label{fig:dist}
% \end{figure}

% \begin{figure}[htbp]
%   \centering
%   \includegraphics[width=0.9\linewidth]{imgs/features_2.png}
%   \caption{The feature visualizations of different time of GM Framework.}
%   \label{fig:features_2}
% \end{figure}






\textbf{Model Merging}.
We evaluate the performance of the model without EMA.
$\mathcal{M}_f$ increases for 55\% and $\mathcal{M}_d$ decreases for 14\%, which demonstrates the necessity of EMA.
We also consider an alternative fuse method which assigns $\phi_S\leftarrow \phi_D^t$ after the update of $\phi_D^t$ by Eq.~\ref{eq:ema}.
$\mathcal{M}_d$ is significantly affected with a decrease of 33\%.
Therefore, we use the fixed $\phi_S$ in this paper.


\textbf{Static-Dynamic Branch}.
The multi-branch aims to maintain known category information and discover novel categories on different branches.
We first evaluate the performance when directly replacing the multi-branch with a single one.
The results show that $\mathcal{M}_f$ increases dramatically, which demonstrates the importance of the multi-branch to preserve already learned categories.
We further investigate the components of the static-dynamic branch.
Removing the initialization of branch $\phi_D^0$ also degrades both $\mathcal{M}_f$ and $\mathcal{M}_d$.
For the proposed loss $\mathcal{L}_{\text{SD}}$ aligning the feature space of  $\phi_S$ and  $\phi_D^t$,
%The performances of the model without $\mathcal{L}_{\text{SD}}$ and the model replacing $\mathcal{L}_{\text{SD}}$ with DINO~\cite{DBLP:conf/iccv/CaronTMJMBJ21} are presented.
%DINO is an alternative of $\mathcal{L}_{\text{SD}}$ which considers the features of the branches after Softmax as the probability distributions and applies the distill loss %cite to make the distributions similar.
results show that the model without $\mathcal{L}_{\text{SD}}$ performs worse on both $\mathcal{M}_f$ and $\mathcal{M}_d$ for the separation of the feature spaces leading to the failure of the prototype mechanism.
The model replacing $\mathcal{L}_{\text{SD}}$ with DINO~\cite{DBLP:conf/iccv/CaronTMJMBJ21} increases $\mathcal{M}_f$ for 3\% and decreases $\mathcal{M}_d$ for 6.3\%.
% Therefore, $\mathcal{L}_{\text{SD}}$ is used in this paper.

\textbf{Sifting in Merging}.
Sifting aims to sift out samples with low cluster confidence given by the cluster head.
Except for the criterion based on the adopted local geometry property, there are several potential criteria to sift samples.
\textit{Confidence Ranking (CR)} selects a portion of all samples with the highest score .
\textit{Conditional Confidence Ranking (CCR)} selects a portion of samples from each class with the highest score.
\textit{Confidence Filtering (CF)} selects the samples with the score higher than a given threshold.
The results show that: (i) For $\mathcal{M}_f$, the model without sifting and CR performs worse, and CCR, CF and the local sample density  based method performs at almost same level. (ii) For $\mathcal{M}_d$, the local sample density  based method outperforms all of these compared methods.








\textbf{Hyperparameter Analysis of Static-Dynamic Branch}.
We also evaluate the effect of $\alpha$ in Eq.~\ref{eq:ema}, shown in Figure~\ref{fig:alpha}.
The hyper-parameter $\alpha$ controls the importance of $\phi_S$ relative to $\phi_D^t$.
For the model with only EMA, both $\mathcal{M}_f$ and $\mathcal{M}_d$ decrease with the increase of $\alpha$, since the model with higher $\alpha$ maintains more information from the known categories.
The model with only $\mathcal{L}_{\text{SD}}$ (\ie, the model w/o. EMA shown in Tabel~\ref{tab:abla:1}) performs worse than the proposed full model, which demonstrates that only the constrain of the distance between the feature space of $\phi_S$ and $\phi_D^t$ is not enough to transfer the knowledge from $\phi_S$ to  $\phi_D^t$.
The performances of the models with both EMA and $\mathcal{L}_{\text{SD}}$ varies smoother, compared with the models with only EMA.
Therefore, the models could achieve higher performances and be more robust by combining EMA and $\mathcal{L}_{\text{SD}}$.

\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.85\linewidth]{imgs/alpha.png}
    \caption{The variation comparison of the performance of the models by varying $\alpha$. \textbf{a}: $\mathcal{M}_f$ of the model with only EMA; \textbf{b}: $\mathcal{M}_d$ of the model with only EMA; \textbf{c}: $\mathcal{M}_f$ of the model with both EMA and $\mathcal{L}_{\text{SD}}$; \textbf{d}: $\mathcal{M}_d$ of the model with both EMA and $\mathcal{L}_{\text{SD}}$.}
    \label{fig:alpha}
\end{figure}





\input{tables/tab_ab}


==> NeurIPS 2022 SMNet_0517_arxiv/sections/chap05_related.tex <==
\section{Related Work}
\label{sec_rel}
\textbf{Novel Class Discovery}~\cite{han2021autonovel,UNO, DBLP:journals/corr/abs-2201-02609,dualrank} aims to discover unknown classes from unlabeled data by leveraging pairwise similarity~\cite{han2021autonovel,joint} or employing unsupervised clustering~\cite{dtc,ncl}. Most of these methods assume that there is a pure unlabeled set that only contains samples from unknown categories, which means the class space of unlabeled data is completely disjoint with the labeled set. And at test time, samples are all from novel classes. These assumptions limit their applications in the real world. CCD aims to tackle novel class discovery under a more realistic situation in which the unlabeled data (i) are continuously confronted and (ii) contain both known and unknown classes.%, which is more realistic than existing scenario.

% \textbf{Semi-supervised Learning} improves the model performance by leveraging unlabeled data which are easy to be obtained in most cases~\cite{zhusslsurvey}. A common assumption in this setting is the labeled data and unlabeled data share the same category space~\cite{EntMin,temporalensembling, mixmatch,Fixmatch}. Recent methods~\cite{ds3l,openmatch,ngc} tackle the situation that unlabeled data contains samples from both known and unknown classes by rejecting unknown-class samples. All of these methods cannot discover potential existed novel classes in unlabeled data. The goal of open-world semi-supervised learning~\cite{owssl} is to classify known classes while discovering unknown classes at the same time. However, it works in a transductive learning setting and assumes there is no incremental unlabeled data. %While in the real world, unlabeled data are continuously confronted, and some of them belong to novel classes. 
% Different from existing novel class discovery, CCD aims to handle the continuous unlabeled data by discovering novel categories from them while leveraging unlabeled data from known classes to improve the model performance.
%CCD aims to deal with the situation in which the unlabeled data (i) are continuously confronted and (ii) contain both known and unknown classes, which is more realistic than existing scenarios.

\textbf{Continual Learning} needs the model to extend its ability to address new tasks when confronted with new data~\cite{continualsurvey,  dualnet,co2,dualaug,liu2022continual,miao2022continual,madaan2022representational,yu2022unlabeled,mohammad2022prob}. The main challenge of continual learning is to avoid catastrophic forgetting~\cite{DBLP:journals/connection/Robins95,goodfellow2013empirical}, \ie, the performance degradation on previously learned tasks when new ones are ingested. Existing methods can be categorized into replay methods~\cite{icarl, dgreplay, gem}, regularization-based methods~\cite{lwf,synaptic,imm} and parameter isolation methods~\cite{packnet, piggyback,rcl}. Most of the methods assume there are available labeled data in each time-step. Nevertheless, the data in continuous streams are more likely to be unlabeled in reality, which means the category information is unknown and needs to be discovered. 
\par
Different from existing novel category discovery and continual learning, CCD requires the model to discover novel categories from the continuous unlabeled data while maintaining the classification performance on known and discovered classes.
% \textbf{Open-set Recognition} deals with samples from unknown classes during testing phase~\cite{osr,osrsurvey}. The model is trained on labeled data, and samples belonging to unknown classes could appear in the testing phase. The model is expected to classify samples from known classes and rejected samples from unknown classes. Open-world Recognition moves beyond just recognizing and rejecting these unknown-class samples and toward making the model have the ability to classify these samples by a designed human-in-the-loop scheme~\cite{owr}. However, the need for annotators limits the application of such methods. On the contrary, CCD needs the model to (i) discover and classify unknown classes automatically from unlabeled data and (ii) handle the continuous unlabeled data.

==> NeurIPS 2022 SMNet_0517_arxiv/sections/chap06_conclusion.tex <==
\section{Conclusion}
\label{sec:concl}
In this paper, we study the continuous category discovery (CCD) problem where unlabeled data are continuously fed into the category discovery system. The main challenge of the CCD problem is that different sets of features are needed to classify known categories and discover novel categories. To address this challenge, we develop a framework called Grow and Merge that alternatively updates the model in the growing phase and the merging phase. Extensive experimental results demonstrate that GM outperforms the existing methods with the less forgetting effect of known categories and higher accuracy for category discovery.

==> NeurIPS 2022 SMNet_0517_arxiv/tables/tab_ab.tex <==

% \begin{minipage}{\textwidth}
% \small
% \centering
%         \begin{minipage}[t]{0.61\textwidth}
%             \centering
%             \makeatletter\def\@captype{table}\makeatother\caption{Experimental results of ablation studies.}
%             %  \renewcommand\arraystretch{1.03}
% \begin{tabular}{@{}llrr@{}}
% \toprule
%                                  &                                      & \multicolumn{1}{l}{$\mathcal{M}_f$ $\downarrow$} & \multicolumn{1}{l}{$\mathcal{M}_d$ $\uparrow$} \\ \midrule
% GM                             &                                      & 9.79                           & 35.77                         \\ \midrule
% %\multirow{2}{*}{Tighten} &
% %{Grow phase} &
% \multirow{3}{*}{Growing phase} &
% WTA+$\mathcal{L}_{\text{SD}}$+CE &  9.51  &  31.50 \\
%                          & WTA+$\mathcal{L}_{\text{SD}}$+SimCLR & 9.69 & 31.47  \\
%   & WTA+$\mathcal{L}_{\text{SD}}$+SimSiam       & 9.51  &    34.07           \\
%                          \midrule
% \multirow{4}{*}{Merging phase}             & CE + PLL                               & 8.89                           & 33.23                         \\
%                                  & CE                                   & 7.41                           & 31.03                         \\
%                                  & SSL + PLL                              & 9.26                           & 32.94                         \\
%                                  & SSL                                  & 7.23                           & 29.03                         \\ \midrule
% \multirow{4}{*}{Static-Dynamic Branch}    & w/o. Multi-Branch                    & 33.23                          & 35.10                         \\
%                                  & w/o. Initialize $\phi_D^0$ & 27.91                          & 31.77                         \\ 
                                 
%                                 %  \midrule
% % \multirow{2}{*}{Static-Dynamic Distillation Loss} 
% & w/o. $\mathcal{L}_{\text{SD}}$                        & 15.41                          & 29.97                         \\
%                                  & DINO                                 & 9.82                           & 33.53                         \\ \midrule
% \multirow{4}{*}{Sifting in the Merging}         & w/o. Sifting                         & 9.83                           & 31.44                         \\
%                                  & Sifting (CR)                         & 9.93                           & 32.46                         \\
%                                  & Sifting (CCR)                        & 9.76                           & 33.76                         \\
%                                  & Sifting (CF)                         & 9.74                           & 31.46                         \\  \midrule
% \multirow{2}{*}{Model Merging}             & w/o. EMA                             & 15.27                          & 30.87                         \\
%                                  & Update $\phi_S$          & 10.67                          & 24.13                         \\
% \bottomrule
% \end{tabular}
% \label{tab:abla}
%         \end{minipage}
%         \hspace{0.35cm}
% \begin{minipage}[t]{0.35\textwidth}
%         \centering
%         \makeatletter\def\@captype{table}\makeatother\caption{Additional study on multi-branch.}
% \begin{tabular}{@{}crrr@{}}
% \toprule
%                         &  $\alpha$    & $\mathcal{M}_f$ $\downarrow$  & $\mathcal{M}_d$ $\uparrow$    \\ \midrule
% \multirow{6}{*}{EMA}    & 0.25 & 17.00    & 31.63     \\
%                         & 0.50  & 16.51 & 30.33 \\
%                         & 0.75 & 16.44 & 31.67     \\
%                         & 0.80  & 15.77 & 31.57 \\
%                         & 0.90  & 16.53 & 30.07 \\
%                         & 0.99 & 15.41 & 29.97 \\ \midrule
% $\mathcal{L}_{\text{SD}}$                      &      & 15.27 & 30.87    \\ \midrule
% \multirow{6}{*}{EMA + $\mathcal{L}_{\text{SD}}$} & 0.25 & 9.61  & 32.67     \\
%                         & 0.50  & 9.50   & 35.17 \\
%                         & 0.75 & 9.79  & 33.83     \\
%                         & 0.80  & 9.63  & 33.03 \\
%                         & 0.90  & 10.23 & 35.23 \\
%                         & 0.99 & 9.79  & 35.77    \\ \bottomrule
% \end{tabular}
% \label{tab:ema-ts}
%         \end{minipage}
%     \end{minipage}
    
    
    
    
    
    
\begin{minipage}{\textwidth}
\scriptsize
% \centering
        \begin{minipage}[t]{0.47\textwidth}
            \centering
            \makeatletter\def\@captype{table}\makeatother\caption{Results of ablation studies on GM phases. (mean$\pm$std.)
%             on Growing phase, Merging phase and Model Merging.
            }
            %  \renewcommand\arraystretch{1.03}
            \resizebox{\textwidth}{!}{%
\begin{tabular}{@{}p{52pt}p{56pt}rr@{}}
\toprule
                                 &                                      & {$\mathcal{M}_f$ $\downarrow$} & {$\mathcal{M}_d$ $\uparrow$} \\ \midrule
GM                             &                                      & 9.87$\pm$0.25                          & 35.97$\pm$1.28                         \\ \midrule
%\multirow{2}{*}{Tighten} &
%{Grow phase} &
\multirow{3}{*}{Growing Phase} &
WTA+$\mathcal{L}_{\text{SD}}$+CE &  9.54$\pm$0.04  &  31.37$\pm$0.19 \\
                         & WTA+$\mathcal{L}_{\text{SD}}$+SimCLR & 9.74$\pm$0.08 & 32.29$\pm$1.42  \\
  & WTA+$\mathcal{L}_{\text{SD}}$+SimSiam       & 9.56$\pm$0.06  &    34.81$\pm$1.06           \\
                         \midrule
\multirow{4}{*}{Merging Phase}             & CE + PLL                               & 8.83$\pm$0.30                           & 34.48$\pm$1.09                         \\
                                 & CE                                   & 7.27$\pm$0.25                           & 31.95$\pm$0.81                         \\
                                 & SSL + PLL                              & 9.19$\pm$0.17                           & 34.94$\pm$2.01                         \\
                                 & SSL                                  & 7.55$\pm$0.28                           & 31.03$\pm$1.82                         \\ \midrule
\multirow{2}{*}{Model Merging}             & w/o. EMA                             & 17.72$\pm$2.12                         & 31.18$\pm$2.15                         \\
                                 & Update $\phi_S$          & 11.75$\pm$1.35                         & 24.34$\pm$2.66                       \\
\bottomrule
\end{tabular}
}
\label{tab:abla:1}
        \end{minipage}
        \hspace{0.35cm}
\begin{minipage}[t]{0.48\textwidth}
        \centering
        \makeatletter\def\@captype{table}\makeatother\caption{Results of ablation studies on Static-Dynamic Branch and Sifting in the Merging. (mean$\pm$std.)}
        \resizebox{\textwidth}{!}{%
\begin{tabular}{@{}llrr@{}}
\toprule
                                 &                                      & {$\mathcal{M}_f$ $\downarrow$} & {$\mathcal{M}_d$ $\uparrow$} \\ \midrule
GM                             &                                     & 9.87$\pm$0.25                          & 35.97$\pm$1.28                         \\ \midrule
%\multirow{2}{*}{Tighten} &
%{Grow phase} &
\multirow{4}{*}{Static-Dynamic Branch}    & w/o. Multi-Branch                    & 33.46$\pm$0.65                         & 33.80$\pm$1.17                        \\
                                 & w/o. Initialize $\phi_D^0$ & 26.91$\pm$1.16                          & 31.81$\pm$2.27                         \\ 
                                 
                                %  \midrule
% \multirow{2}{*}{Static-Dynamic Distillation Loss} 
& w/o. $\mathcal{L}_{\text{SD}}$                        & 15.78$\pm$0.42                         & 31.71$\pm$1.88                         \\
                                 & DINO                                 & 9.58$\pm$0.30                        & 32.89$\pm$1.24                         \\ \midrule
\multirow{4}{*}{Sifting in the Merging}         & w/o. Sifting                         & 10.00$\pm$0.15                           & 31.68$\pm$0.45                         \\
                                 & Sifting (CR)                         & 9.91$\pm$0.19                           & 33.18$\pm$1.46                         \\
                                 & Sifting (CCR)                        & 9.74$\pm$0.58                           & 32.86$\pm$0.95                         \\
                                 & Sifting (CF)                         & 9.78$\pm$0.06                           & 31.93$\pm$0.66                         \\ 
\bottomrule
\end{tabular}
}
\label{tab:abla:2}
        \end{minipage}
    \end{minipage}

==> NeurIPS 2022 SMNet_0517_arxiv/tables/tab_ci.tex <==

% 大概改了下数据表格的排版方式，可参考
% \begin{table}[]
% \small
% \centering
% \caption{Experimental results under CI scenario (mean$\pm$std.).}
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{@{}lrrrrrrrrrrrr@{}}
% \toprule
%                                 & \multicolumn{2}{c}{\textbf{CIFAR-100}} & \multicolumn{2}{c}{\textbf{CUB-200}} & \multicolumn{2}{c}{\textbf{ImageNet-100}} & \multicolumn{2}{c}{\textbf{Stanford-Cars}} & \multicolumn{2}{c}{\textbf{FGVC-Aircraft}} & \multicolumn{2}{c}{\textbf{ImageNet-200}}\\
%           Method                     & $\mathcal{M}_f$ $\downarrow$     & $\mathcal{M}_d$ $\uparrow$    & $\mathcal{M}_f$ $\downarrow$  & $\mathcal{M}_d$ $\uparrow$   & $\mathcal{M}_f$  $\downarrow$    & $\mathcal{M}_d$  $\uparrow$ & $\mathcal{M}_f$ $\downarrow$     & $\mathcal{M}_d$ $\uparrow$ & $\mathcal{M}_f$ $\downarrow$     & $\mathcal{M}_d$ $\uparrow$ & $\mathcal{M}_f$ $\downarrow$     & $\mathcal{M}_d$ $\uparrow$    \\ \midrule
% \textit{lower-bound of $\mathcal{M}_f$ (offline K-Means)~\cite{kmeans}}  & 5.37$\pm$0.70 & 16.95$\pm$1.04 &  2.94$\pm$1.03 & 14.29$\pm$0.47  &  3.03$\pm$5.47 & 18.20$\pm$0.58 & 2.41$\pm$0.59 & 10.23$\pm$0.32 & 3.86$\pm$0.71 & 15.10$\pm$1.25 & 3.16$\pm$0.76 & 15.28$\pm$0.67 \\
% \textit{upper-bound of $\mathcal{M}_d$ (offline AutoNovel)~\cite{han2021autonovel}} & 5.12$\pm$0.84            & 42.27$\pm$4.97        & 7.57$\pm$0.77      & 16.13$\pm$0.37       & 6.81$\pm$0.98          & 34.18$\pm$1.77       & 11.24$\pm$0.59 & 20.69$\pm$3.28 & 6.95$\pm$2.40 & 27.67$\pm$0.86 &  5.98$\pm$0.67 & 24.62$\pm$0.47  \\ 
% \midrule
% AutoNovel (online)~\cite{han2021autonovel}                       & 66.76$\pm$1.56          & 29.65$\pm$4.60        & 60.66$\pm$0.20       & 18.08$\pm$0.84       &     63.00$\pm$0.42        &      5.83$\pm$1.81 & 72.07$\pm$0.17 & 16.71$\pm$1.40  & 53.23$\pm$0.60 & 26.93$\pm$1.48 & 60.79$\pm$0.61 & 10.21$\pm$2.52  \\
% DRNCD (online)~\cite{drncd}                  & 64.99$\pm$1.89         & 8.53$\pm$2.35       & 42.74$\pm$0.28        & 6.30$\pm$0.93      &       47.02$\pm$2.18          &    5.00$\pm$1.37  & 50.70$\pm$3.29 & 2.39$\pm$0.84 & 38.89 $\pm$4.15& 5.35$\pm$0.07    &  43.91$\pm$1.37 & 4.39$\pm$1.20  \\
% AutoNovel (online) + LwF~\cite{han2021autonovel, lwf}  & 23.94$\pm$1.54 & 27.84$\pm$0.57 &  59.82$\pm$0.58 & 23.23$\pm$4.81  &  61.31$\pm$0.37 & 7.59$\pm$0.55  & 71.52$\pm$0.33 & 20.31$\pm$0.69  & 44.63$\pm$1.37 & 8.68$\pm$5.67 & 61.03$\pm$0.37 & 9.77$\pm$1.00  \\
% DRNCD (online)  + LwF~\cite{drncd, lwf} & 26.87$\pm$0.15 & 3.57$\pm$0.61 & 45.25$\pm$0.37 & 5.78$\pm$0.51 & 30.88$\pm$1.57 & 6.78$\pm$1.16 & 27.40$\pm$0.50 & 3.88$\pm$0.63 & 38.89$\pm$4.15 &  5.61$\pm$3.00 &  27.40$\pm$0.84 & 6.71$\pm$1.55 \\
% iCaRL (fixed exemplars) + LwF~\cite{icarl,lwf} & 34.79$\pm$0.29 &  - & 42.02$\pm$0.31 & - & 10.04$\pm$0.28 & - &24.31$\pm$0.64 & -  & 22.60$\pm$1.19 & - & 10.55$\pm$0.52& -\\
% \textbf{GM (Ours)}                           & \textbf{9.87$\pm$0.25}           & \textbf{35.97$\pm$1.28}        & \textbf{19.46$\pm$1.63}        & \textbf{24.97$\pm$1.81}       &         \textbf{8.30$\pm$0.42}        &    \textbf{27.24$\pm$0.83}     & \textbf{17.66$\pm$0.70} &\textbf{25.77$\pm$0.54}  & \textbf{8.21$\pm$0.27} & \textbf{29.65$\pm$1.63}   & \textbf{7.50$\pm$1.60}  & \textbf{19.33$\pm$0.46} \\ \bottomrule
% \end{tabular}
% }
% \label{tab:ci}
% \end{table}

\begin{table*}[]
\small
\centering
\caption{Experimental results under CI scenario (mean$\pm$std.).}
\resizebox{1\textwidth}{!}{%
\begin{tabular}{@{}lrrrrrr@{}}
\toprule
                                & \multicolumn{2}{c}{\textbf{CIFAR-100}} & \multicolumn{2}{c}{\textbf{CUB-200}} & \multicolumn{2}{c}{\textbf{ImageNet-100}} \\
          Method                     & $\mathcal{M}_f$ $\downarrow$     & $\mathcal{M}_d$ $\uparrow$    & $\mathcal{M}_f$ $\downarrow$  & $\mathcal{M}_d$ $\uparrow$   & $\mathcal{M}_f$  $\downarrow$    & $\mathcal{M}_d$  $\uparrow$   \\ \midrule
\textit{lower-bound of $\mathcal{M}_f$ (offline K-Means)}  & 5.37$\pm$0.70 & 16.95$\pm$1.04 &  2.94$\pm$1.03 & 14.29$\pm$0.47  &  3.03$\pm$5.47 & 18.20$\pm$0.58  \\
\textit{upper-bound of $\mathcal{M}_d$ (offline AutoNovel)} & 5.12$\pm$0.84            & 42.27$\pm$4.97        & 7.57$\pm$0.77      & 16.13$\pm$0.37       & 6.81$\pm$0.98          & 34.18$\pm$1.77         \\ 
\midrule
AutoNovel (online)                     & 66.76$\pm$1.56          & 29.65$\pm$4.60        & 60.66$\pm$0.20       & 18.08$\pm$0.84       &     63.00$\pm$0.42        &      5.83$\pm$1.81   \\
DRNCD (online)                & 64.99$\pm$1.89         & 8.53$\pm$2.35       & 42.74$\pm$0.28        & 6.30$\pm$0.93      &       47.02$\pm$2.18          &    5.00$\pm$1.37    \\
AutoNovel (online) + LwF  & 23.94$\pm$1.54 & 27.84$\pm$0.57 &  59.82$\pm$0.58 & 23.23$\pm$4.81  &  61.31$\pm$0.37 & 7.59$\pm$0.55    \\
DRNCD (online)  + LwF & 26.87$\pm$0.15 & 3.57$\pm$0.61 & 45.25$\pm$0.37 & 5.78$\pm$0.51 & 30.88$\pm$1.57 & 6.78$\pm$1.16 \\
iCaRL (fixed exemplars) + LwF & 34.79$\pm$0.29 &  - & 42.02$\pm$0.31 & - & 10.04$\pm$0.28 & - \\
\textbf{GM (Ours)}                           & \textbf{9.87$\pm$0.25}           & \textbf{35.97$\pm$1.28}        & \textbf{19.46$\pm$1.63}        & \textbf{24.97$\pm$1.81}       &         \textbf{8.30$\pm$0.42}        &    \textbf{27.24$\pm$0.83}  \\ \bottomrule
%
\toprule
                                & \multicolumn{2}{c}{\textbf{Stanford-Cars}} & \multicolumn{2}{c}{\textbf{FGVC-Aircraft}} & \multicolumn{2}{c}{\textbf{ImageNet-200}}\\
          Method                     & $\mathcal{M}_f$ $\downarrow$     & $\mathcal{M}_d$ $\uparrow$    & $\mathcal{M}_f$ $\downarrow$  & $\mathcal{M}_d$ $\uparrow$   & $\mathcal{M}_f$  $\downarrow$    & $\mathcal{M}_d$  $\uparrow$     \\ \midrule
\textit{lower-bound of $\mathcal{M}_f$ (offline K-Means)}  &  2.41$\pm$0.59 & 10.23$\pm$0.32 & 3.86$\pm$0.71 & 15.10$\pm$1.25 & 3.16$\pm$0.76 & 15.28$\pm$0.67 \\
\textit{upper-bound of $\mathcal{M}_d$ (offline AutoNovel)}  & 11.24$\pm$0.59 & 20.69$\pm$3.28 & 6.95$\pm$2.40 & 27.67$\pm$0.86 &  5.98$\pm$0.67 & 24.62$\pm$0.47  \\ 
\midrule
AutoNovel (online)                    & 72.07$\pm$0.17 & 16.71$\pm$1.40  & 53.23$\pm$0.60 & 26.93$\pm$1.48 & 60.79$\pm$0.61 & 10.21$\pm$2.52  \\
DRNCD (online)                 & 50.70$\pm$3.29 & 2.39$\pm$0.84 & 38.89 $\pm$4.15& 5.35$\pm$0.07    &  43.91$\pm$1.37 & 4.39$\pm$1.20  \\
AutoNovel (online) + LwF    & 71.52$\pm$0.33 & 20.31$\pm$0.69  & 44.63$\pm$1.37 & 8.68$\pm$5.67 & 61.03$\pm$0.37 & 9.77$\pm$1.00  \\
DRNCD (online)  + LwF  & 27.40$\pm$0.50 & 3.88$\pm$0.63 & 38.89$\pm$4.15 &  5.61$\pm$3.00 &  27.40$\pm$0.84 & 6.71$\pm$1.55 \\
iCaRL (fixed exemplars) + LwF  &24.31$\pm$0.64 & -  & 22.60$\pm$1.19 & - & 10.55$\pm$0.52& -\\
\textbf{GM (Ours)}                             & \textbf{17.66$\pm$0.70} &\textbf{25.77$\pm$0.54}  & \textbf{8.21$\pm$0.27} & \textbf{29.65$\pm$1.63}   & \textbf{7.50$\pm$1.60}  & \textbf{19.33$\pm$0.46} \\ \bottomrule
\end{tabular}
}
\label{tab:ci}
\end{table*}

==> NeurIPS 2022 SMNet_0517_arxiv/tables/tab_scenarios.tex <==
\begin{table}[htbp]
\small
\centering
\caption{The content of $\mathcal{D}_{train}^t$ under different scenarios DI, CI,  MI and SMI.}
\begin{tabular}{@{}ccccc@{}}
\toprule
   & Known Categories & Novel Categories  & Labeled data  & Unlabeled data \\ \midrule
CI &                          \XSolidBrush                       &                     \Checkmark       &     \XSolidBrush            &                     \Checkmark        \\
DI &                        \Checkmark                     &              \XSolidBrush        &        \XSolidBrush                 &                     \Checkmark    \\
MI &                      \Checkmark                         &                   \Checkmark       &       \XSolidBrush       &                     \Checkmark           \\ 
SMI &  \Checkmark & \Checkmark & \Checkmark &                     \Checkmark    \\ \bottomrule
\end{tabular}
\label{tab:scenario}
\end{table}

==> checklist.tex <==
\section*{Checklist}



\begin{enumerate}


\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{} See supplementary materials.
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{} See supplementary materials.
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}


\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{} Theoretical results are not included.
        \item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}


\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{} See the supplementary materials.
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{} See section~\ref{sec:exp} and supplementary materials.
        \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerNo{}
        \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{} See supplementary materials.
\end{enumerate}


\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{} See Section~\ref{sec:exp}.
  \item Did you mention the license of the assets?
    \answerNA{} The license of the assets are not provided on their official website.
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNo{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNo{}
\end{enumerate}


\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{} Crowdsourcing and human subjects are not used in this research.
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}


\end{enumerate}
